Trace-Guided Synthesis of Effectful Test Generators

Several recently proposed program logics have incorporated notions of underapproximation into their design, enabling them to reason about reachability rather than safety. In this paper, we explore how similar ideas can be integrated into an expressive type and effect system. We use the resulting underapproximate type specifications to guide the synthesis of test generators that probe the behavior of effectful black-box systems. A key novelty of our type language is its ability to capture underapproximate behaviors of effectful operations using symbolic traces that expose latent data and control dependencies, constraints that must be preserved by the test sequences the generator outputs. We implement this approach in a tool called Clouseau, and evaluate it on a diverse range of applications by integrating Clouseau's synthesized generators into property-based testing frameworks like QCheck and model-checking tools like P. In both settings, the generators synthesized by Clouseau are significantly more effective than the default testing strategy, and are competitive with state-of-the-art, handwritten solutions.

==> Makefile <==
.PHONY: haste all clean cleanall nocite clouseau

DEPS = main.tex bibliography.bib commands.sty refinementtydef.sty \
	sections/0-intro.tex sections/1-overview.tex sections/2-language.tex \
	sections/3-algo.tex sections/4-evaluation.tex sections/5-related.tex \
	tech/outlines.tex tech/0-semantics.tex tech/1-typing.tex tech/2-denotation.tex \
	tech/3-algo.tex tech/4-proof-0.tex tech/5-explanation.tex tech/6-evaluation.tex

all: clouseau.pdf clouseau-diff.pdf clouseau-sm-full.pdf

clouseau: clouseau.pdf

clouseau.pdf: $(DEPS)
	pdflatex -jobname="clouseau" -shell-escape main
	bibtex clouseau
	pdflatex -jobname="clouseau" -shell-escape main
	pdflatex -jobname="clouseau" -shell-escape main

clouseau-diff.pdf: $(DEPS)
	pdflatex -jobname="clouseau-diff" -shell-escape "\def\diffmode{}\input main.tex"
	bibtex clouseau-diff
	pdflatex -jobname="clouseau-diff" -shell-escape "\def\diffmode{}\input main.tex"
	pdflatex -jobname="clouseau-diff" -shell-escape "\def\diffmode{}\input main.tex"

clouseau-sm-full.pdf: $(DEPS)
	pdflatex -jobname="clouseau-sm-full" -shell-escape "\def\showappendix{true}\input main.tex"
	bibtex clouseau-sm-full
	pdflatex -jobname="clouseau-sm-full" -shell-escape "\def\showappendix{true}\input main.tex"
	pdflatex -jobname="clouseau-sm-full" -shell-escape "\def\showappendix{true}\input main.tex"

clouseau-sm-techreport.pdf: $(DEPS)
	pdflatex -jobname="clouseau-sm-techreport" -shell-escape "\def\techreportmode{true}\def\showappendix{true}\input main.tex"
	bibtex clouseau-sm-techreport
	pdflatex -jobname="clouseau-sm-techreport" -shell-escape "\def\techreportmode{true}\def\showappendix{true}\input main.tex"
	pdflatex -jobname="clouseau-sm-techreport" -shell-escape "\def\techreportmode{true}\def\showappendix{true}\input main.tex"

# create pdf without bibs (fast)
haste:
	pdflatex -jobname="clouseau" -shell-escape main

# remove tex objects
clean:
	rm -f *.log *.aux *.blg *.bbl *.out *~ *.cut sections/*.aux sections/tech/*.aux *.cb *.cb2

# remove objects, including the pdf file
cleanall:
	rm -f *.log *.aux *.blg *.bbl *.out *~ *.cut sections/*.aux sections/tech/*.aux *.cb *.cb2 *.pdf

# check for things in the bib that aren't cited/used
# and citations in the file that aren't in the bib
nocite:
	checkcites clouseau

